LegalVis: Exploring and Inferring Precedent Citations in Legal Documents

To reduce the number of pending cases and conflicting rulings in the Brazilian Judiciary, the National Congress amended the Constitution, allowing the Brazilian Supreme Court (STF) to create binding precedents (BPs), i.e., a set of understandings that both Executive and lower Judiciary branches must follow. The STF's justices frequently cite the 58 existing BPs in their decisions, and it is of primary relevance that judicial experts could identify and analyze such citations. To assist in this problem, we propose LegalVis, a web-based visual analytics system designed to support the analysis of legal documents that cite or could potentially cite a BP. We model the problem of identifying potential citations (i.e., non-explicit) as a classification problem. However, a simple score is not enough to explain the results; that is why we use an interpretability machine learning method to explain the reason behind each identified citation. For a compelling visual exploration of documents and BPs, LegalVis comprises three interactive visual components: the first presents an overview of the data showing temporal patterns, the second allows filtering and grouping relevant documents by topic, and the last one shows a document's text aiming to interpret the model's output by pointing out which paragraphs are likely to mention the BP, even if not explicitly specified. We evaluated our identification model and obtained an accuracy of 96%; we also made a quantitative and qualitative analysis of the results. The usefulness and effectiveness of LegalVis were evaluated through two usage scenarios and feedback from six domain experts.

==> makefile <==
# --------------------------------------------------------------------
# Usage:
#
#	all	 make pdf file
#	pdf	 make pdf file
#	clean	 remove files
#	clobber  remove everything
#	check	 doubled word and latex syntax check
#	wc	 word count
# --------------------------------------------------------------------

NAME := paper
APPENDIX := supp
BIBFILES := paper.bib
TEXFILES := paper.tex

DISTILLER := ps2pdf

# --------------------------------------------------------------------

SHELL := bash
LATEX := pdflatex
BIBTEX := bibtex -min-crossrefs=100 # avoid separating out crossrefs
DETEX := detex -n
LACHECK := lacheck
DW := dw # ftp://ftp.math.utah.edu/pub/misc/dw.tar.gz
RM := rm -f
WC := wc

# --------------------------------------------------------------------

all: $(NAME).pdf 
pdf: $(NAME).pdf
check: dw syn

$(NAME).pdf: $(NAME).tex $(BIBFILES) 
	@echo '-------------------- latex appendix --------------'
	$(LATEX) $(APPENDIX).tex 
	@echo '-------------------- latex appendix --------------'
	$(LATEX) $(APPENDIX).tex
	@echo '-------------------- latex #1 --------------------'
	$(LATEX) $(NAME).tex
	@echo '-------------------- bibtex --------------------'
	$(BIBTEX) $(NAME)
	@echo '-------------------- latex #2 --------------------'
	$(LATEX) $(NAME).tex
	@echo '-------------------- latex #3 --------------------'
	$(LATEX) $(NAME).tex

dw:
	@-$(RM) $(NAME).dw
	@echo '-------------------- doubled words --------------------'
	@for f in $(NAME).tex ;\
	do \
		echo ----- $$f ----- ; \
		echo ----- $$f ----- >> $(NAME).dw ; \
		$(DETEX) $$f  | $(DW) >> $(NAME).dw ; \
	done

syn:
	@echo '-------------------- syntax check --------------------'
	@$(LACHECK) $(NAME).tex

wc:
	@$(DETEX) $(NAME).tex | $(WC)

clean:
	$(RM) *.{blg,dvi,dw,ilg,log,o,tmp,lbl,aux,bbl,lbl}
	$(RM) *.{idx,ind,toc,lof,lot,brf,out,fls,fdb_latexmk,synctex.gz}
	$(RM) $(NAME).pdf
	$(RM) $(APPENDIX).pdf

clobber: clean
	$(RM) *~ \#* core

